EPIC: Generative AI Platform for Accelerating HPC Operational Data Analytics

We present EPIC, an AI-driven platform designed to augment operational data analytics. EPIC employs a hierarchical multi-agent architecture where a top-level large language model provides query processing, reasoning and synthesis capabilities. These capabilities orchestrate three specialized low-level agents for information retrieval, descriptive analytics, and predictive analytics. This architecture enables EPIC to perform HPC operational analytics on multi-modal data, including text, images, and tabular formats, dynamically and iteratively. EPIC addresses the limitations of existing HPC operational analytics approaches, which rely on static methods that struggle to adapt to evolving analytics tasks and stakeholder demands. Through extensive evaluations on the Frontier HPC system, we demonstrate that EPIC effectively handles complex queries. Using descriptive analytics as a use case, fine-tuned smaller models outperform large state-of-the-art foundation models, achieving up to 26% higher accuracy. Additionally, we achieved 19x savings in LLM operational costs compared to proprietary solutions by employing a hybrid approach that combines large foundational models with fine-tuned local open-weight models.

==> EPIC_arXiv/figs/design_document_module.tex <==
%% Template for a page-wide figure
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/docrag2.png}
    \caption{The Document-RAG module: (a) Ingestion pipeline, and (b) Inference pipeline}
  %\Description{Description of the image}
  \label{figs: document_module}
\end{figure}


==> EPIC_arXiv/figs/design_prediction_module.tex <==
%% Template for a page-wide figure
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/prediction_diagram.png}
  \caption{Predictive Analytics Module, showing the interaction between the Large Language Model (LLM), Prediction model, and user interface for generating predictions and visualizations from natural language queries.}
  %\Description{Description of the image}
  \label{figs:prediction_diagram}
\end{figure}


==> EPIC_arXiv/figs/design_telemetry_module.tex <==
%% Template for a page-wide figure
\begin{figure}[t]
  \centering
  
  \includegraphics[width=\linewidth]{figs/telemetry_flow_diagram.png}
  \caption{Descriptive Analytics module. The inference pipeline is shown by components in blue outline. The auxiliary pipeline (shown in green) is used in evaluation.}
  %\Description{Description of the image}
  \label{fig:telemetry_module_diagram}
\end{figure}


==> EPIC_arXiv/figs/framework.tex <==
%%
%% EPIC: End-to-end architecture
%% 
%% Google Slides path: https://docs.google.com/presentation/d/1PvQIL0uaekQUVevOJ1lYTDJ_nz-f72U24mZIdy09uzM/edit?usp=sharing
%% 
\begin{figure*}[t]
  \centering
  %\includegraphics[width=18cm, height=6cm]{EPIC/figs/epic_arch.pdf}
  \includegraphics[width=18cm, height=6cm]{figs/epic-architecture-v2.pdf}
  \caption{Architecture of the AI assisted data exploration system}
  %\Description{Description of the image}
  \label{figs:architecture}
\end{figure*}


==> EPIC_arXiv/figs/sql_comparision.tex <==
%% Template for a page-wide figure
\begin{figure}[t]
  \centering
  
  \includegraphics[width=\linewidth]{EPIC/figs/sql_comparision.png}
  \caption{The two SQL statements (a) and (b) generate exactly same data despite being different.}
  %\Description{Description of the image}
  \label{fig:sql_comparision}
\end{figure}


==> EPIC_arXiv/tables/document_RAG_human_eval.tex <==
\begin{table}
  \caption{Human and LLM-as-judge Evaluation}
  \label{tab:human-llm-eval}
  %% Footnotesize if a much smaller font is needed
  %\small
  \footnotesize
  \addtolength{\tabcolsep}{-0.4em}
  \centering
  \begin{tabular}{ccccc}
    
    \toprule
      \textbf{Participant} & \textbf{Relevance} & \textbf{Coherence} &  \textbf{Fac. Accuracy} & \textbf{Completeness}\\
     
    \midrule
      SME & 3.92 & 4.15 & 3.65 & 3.76 \\
     
    %\midrule

    GPT-4o & 4.19 & 4.18 & 3.74 & 3.41 \\
     
    
  \bottomrule
\end{tabular}
\end{table}

==> EPIC_arXiv/tables/document_RAG_text.tex <==

% \begin{table*}[]
% \label{tab: doceval}
%     \caption{Evaluation of the document module via Lexical, Semantic, Hallucination metrics}
%     %\footnotesize
%     \centering
%     \addtolength{\tabcolsep}{-0.1em}
%     \begin{tabular}{cccccc|cccc|c}
%         \toprule
%         \multicolumn{6}{c}{\textbf{Lexical}} & \multicolumn{4}{c}{\textbf{Semantic}} & \textbf{Hallucination } \\
%         \multicolumn{6}{c}{{(higher better)}} & \multicolumn{4}{c}{{(higher better; except BARTScore)}} & {(lower better)} \\
%         \cline{1-11}
%         \multicolumn{3}{c}{\textbf{Rouge1}} & \multicolumn{3}{c|}{\textbf{RougeL}} & \multicolumn{3}{c}{\textbf{BERT}} & \multirow{2}{*}{\textbf{BART}} & \multirow{2}{*}{\textbf{SelfCheckGPT-NLI}} \\
%         %\cline{1-9}
%         {F1} & {Precision} & {Recall} & {F1} & {Precision} & {Recall} & {F1} & {Precision} & {Recall} & & \\
%         \midrule
%         0.46 & 0.55 & 0.39 & 0.35 & 0.42 & 0.30 & 0.62 & 0.70 & 0.56 & -4.12 & 0.45 \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:doceval}
% \end{table*}

\begin{table}[]
    \caption{Evaluation of the document module via Lexical, Semantic, Hallucination metrics}
    \label{tab:eval}
    \scriptsize
    \centering
    \addtolength{\tabcolsep}{2em}
    \begin{tabular}{l l c}
        \hline
        \textbf{Category} & \textbf{Metric} & \textbf{Value} \\
        \hline
        \multicolumn{3}{c}{\textbf{Lexical} (higher better)} \\
        \hline
        \quad Rouge1 & F1 & \color{red}{0.58} \\
        & Precision & \color{red}{0.55} \\
        & Recall & \color{red}{0.62} \\
        \cline{2-3}
        \quad RougeL & F1 & \color{red}{0.50} \\
        & Precision & \color{red}{0.47} \\
        & Recall & \color{red}{0.53} \\
        \hline
        \multicolumn{3}{c}{\textbf{Semantic} (higher better; except BARTScore)} \\
        \hline
        \quad BERT & F1 & \color{red}{0.66} \\
        & Precision & \color{red}{0.72} \\
        & Recall & \color{red}{0.58} \\
        \cline{2-3}
        & BART & \color{red}{-2.39} \\
        \hline
        \multicolumn{3}{c}{\textbf{Hallucination} (lower better)} \\
        \hline
        & SelfCheckGPT-NLI & \color{red}{0.33} \\
        \hline
    \end{tabular}
    \label{tab:doceval}
\end{table}


==> EPIC_arXiv/tables/document_rag_table_and_images.tex <==
\begin{table}
  \caption{Table and Image Retrieval Performance}
  \label{tab:table-image-retrieval}
  %% Footnotesize if a much smaller font is needed
  \footnotesize
  \centering
  \begin{tabular}{ccccc}
    
    \toprule
      \textbf{Modality} & \textbf{Top-1 Accuracy} & \textbf{MAP}   \\
    \midrule
      Image & 0.68 & 0.72  \\
     
    
    \midrule

Table & \color{red}{0.66} & \color{red}{0.68}  \\
     
    
  \bottomrule
\end{tabular}
\end{table}

==> EPIC_arXiv/tables/models_and_data.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
    \caption{EPIC: Software, Models and Data}
    \label{tab:models_data}
    \footnotesize
    \addtolength{\tabcolsep}{-0.2em}
    %\scriptsize
    %\begin{tabular}{@{}ll@{}}
    %\begin{tabular}{p{18mm}p{62mm}}
    \begin{tabular}{ll}
        \toprule
        %\hline
        % \multicolumn{2}{c}{\textbf{(a)~Application}} \\ \hline
        % {(i)~Tools}    & Mulit-modal UI, User Document, Telemetry, Prediction \\ %\hline
        % {(ii)~Models}      & List of base LLM models and DL method for prediction \\ %\hline
        % {(iii)~Tools}    & Mulit-modal UI, User Document, Telemetry, Prediction \\ %\hline
        % {(iv)~Models}      & List of base LLM models and DL method for prediction \\ \hline
        
        %\multicolumn{2}{c}{\textbf{(b)~Evaluation Data}} \\ %\hline
        \textbf{Dataset} & \textbf{Description}\\
        \midrule
        {(i)~\textit{IR} Module}          & Expert vetted, gold-standard set of 1000 Q\&A from \\
        & the OLCF documents, manuals, Wikis, and articles.\\% \hline
        {(ii)~\textit{DA} Module}       & About 500 pairs of english language and SQL queries. \\
        &Database schema of Frontier telemetry data. \\
        & Generated telemetry data for evaluating the \textit{DA} module.\\
        {(iii)~\textit{PA} Module}      & (a) Vetted 100 prediction Q\&A  (in 'json' format). \\  
        & (b)Regression models evaluated on Frontier data,\\ 
        & 1-year jobs log containing about 0.5 million jobs. \\ 
        {(iv)~Top-level}  & 
        Generated $181$ data points for the agentic routing \\
        ~\textit{QP} Module & and synthesis evaluation. \\
        \bottomrule        
                                            
    \end{tabular}
    %\vspace{-2mm}
\end{table}

==> EPIC_arXiv/tables/prediction_output_feature.tex <==
\begin{table}[h]
  \caption{Summarized description of the 16 output features predicted by the \texttt{regression} submodule}
  \label{tab:prediction_feature_summary}
  %% Footnotesize if a much smaller font is needed
  %\footnotesize
  \centering
  \scriptsize
  \begin{tabular}{lp{5cm}}
    
    \hline
 \textbf{Features}                   & \textbf{Description}\\                                            \hline
 \multicolumn{2}{c}{\textbf{(a)~Power}} \\ \hline
Node: Max, Mean, Stddev    & Max/Mean/Stddev of the average node power of each node  \\
         GPU:   Max, Mean, Stddev   & Max/Mean/Stddev of the average GPU power of each node   \\
        CPU Memory Max          & Max of the average CPU memory power of each node        \\ \hline
\multicolumn{2}{c}{\textbf{(b)~Temperature}} \\ \hline
Node: Max, Stddev          & Max/Stddev of the average node temperature of each node \\\hline
 \multicolumn{2}{c}{\textbf{(c)~Energy}} \\ \hline
Total: Node,GPU,CPU Memory & Total Node/GPU/CPU Memory Energy consumed               \\
            Node:   Max, Mean          & Max/Mean of the total node energy of each node          \\
            GPU:   Max, Mean           & Max/Mean of the total GPU energy of each node  \\
\hline
\end{tabular}
\end{table}

==> EPIC_arXiv/tables/predictive_eval.tex <==

\begin{table}
  \caption{Evaluation of \textit{PA} \texttt{regression} submodule for Test Set}
  \label{tab:prediction_regression}
  %% Footnotesize if a much smaller font is needed
  %\footnotesize
  \scriptsize
  \centering
  \begin{tabular}{ccccc}
    
    \toprule
      \textbf{Output Features}&\textbf{MAE} & \textbf{RMSE} & \textbf{MAPE}  \\
    \midrule
    %1.54E+06	6.93E+03	0.11
      GPU Power Max        & 133.60   & 67.23    & 0.35 \\
GPU Power Mean       & 177.01   & 66.38    & 0.34 \\
CPU Memory Power Max & 8.33     & 4.84     & 0.06 \\
Node Power Mean      & 7263.45  & 368.99   & 0.29 \\
Node Temperature Max & 8.96     & 4.58     & 0.08 \\
Total Node Energy        & 9.93E+10 & 6.43E+08 & 0.33 \\
Node Energy Mean     & 2.78E+08 & 1.54E+06 & 0.31 \\
CPU Memory Energy    & 5.08E+07 & 1.32E+06 & 0.12\\

    
  \bottomrule
\end{tabular}
\end{table}

==> EPIC_arXiv/tables/routing_eval.tex <==
\begin{table}
  \caption{\woong~Evaluation of Routing, Reasoning and Synthesis}
  \label{tab:routing_eval}
  %% Footnotesize if a much smaller font is needed
  %\footnotesize
  \centering
  \begin{tabular}{ccccc}
    
    \toprule
      colA & colB & colC & colD  \\
    \midrule
      \multirow{3}{*}{\rotatebox{90}{\parbox{1cm}{\centering Query Parsing}}}& \O & 1 in 1,000 & hello  & world  \\
      & \O & 1 in 1,000 & hello  & world  \\
      & \O & 1 in 1,000 & hello  & world  \\
    
    \midrule

  \multirow{3}{*}{\rotatebox{90}{\parbox{1cm}{\centering Prediction model}}}& \O & 1 in 1,000 & hello  & world  \\
      & \O & 1 in 1,000 & hello  & world  \\
      & \O & 1 in 1,000 & hello  & world  \\
    
  \bottomrule
\end{tabular}
\end{table}

==> EPIC_arXiv/tables/telemetry_eval.tex <==
\begin{table}
      \caption{Evaluation of the telemetry results based on the complexity by SQL functions.}
      \label{tab:telemetry_results_key_fun}
    \scriptsize
    %\footnotesize
    \addtolength{\tabcolsep}{-0.4em}
    \begin{tabular}{llcc}
    \toprule

         & \textbf{{SQL Functions \& Keywords}} & \textbf{All} & \textbf{Correct} \\
            \midrule
        0 & AVERAGE, MAX, JOIN, GROUP BY & 11 & 8 \\
        1 & CASE WHEN, COUNT, GROUP BY, NEW COLUMN & 11 & 8 \\
        2 & COUNT, AVERAGE, EXTRACT, JOIN, GROUP BY & 11 & 10 \\
        3 & COUNT, DISTINCT & 7 & 6 \\
        4 & COUNT, FRACTION, WHERE & 11 & 11 \\
        5 & COUNT, FRACTION, WHERE, JOIN, CASE WHEN, GROUP BY & 11 & 9 \\
        6 & COUNT, JOIN, GROUP BY & 31 & 27 \\
        7 & COUNT, JOIN, WHERE, GROUP BY & 24 & 22 \\
        8 & COUNT, JOIN, WHERE, GROUP BY, ORDER BY & 22 & 20 \\
        9 & COUNT, WHERE & 11 & 11 \\
        10 & DATE\_TRUNC, AVERAGE, JOIN, GROUP BY & 11 & 11 \\
        11 & DATE\_TRUNC, AVERAGE, JOIN, GROUP BY, ORDER BY & 22 & 17 \\
        12 & DATE\_TRUNC, AVERAGE, MAX, WHERE, GROUP BY, ORDER BY & 11 & 11 \\
        13 & DATE\_TRUNC, COUNT, GROUP BY & 11 & 11 \\
        14 & DATE\_TRUNC, COUNT, GROUP BY, ORDER BY & 22 & 21 \\
        15 & DATE\_TRUNC, COUNT, JOIN, GROUP BY & 11 & 11 \\
        16 & DATE\_TRUNC, COUNT, JOIN, WHERE, GROUP BY, ORDER BY & 11 & 11 \\
        17 & DATE\_TRUNC, COUNT, WHERE, GROUP BY & 11 & 11 \\
        18 & DATE\_TRUNC, MAX, GROUP BY & 22 & 19 \\
        19 & DATE\_TRUNC, SUM, JOIN, GROUP BY & 11 & 10 \\
        20 & DATE\_TRUNC, SUM, JOIN, GROUP BY, ORDER BY & 11 & 11 \\
        21 & DATE\_TRUNC, WHERE, GROUP BY & 11 & 10 \\
        22 & DISTINCT & 9 & 8 \\
        23 & EXTRACT, AVERAGE, WHERE, DATE\_TRUNC, GROUP BY & 11 & 1 \\
        24 & JOIN, GROUP BY, ORDER BY & 22 & 22 \\
        25 & SUM, FRACTION, JOIN, GROUP BY & 11 & 0 \\
        26 & SUM, GROUP BY & 33 & 29 \\
        27 & SUM, JOIN, GROUP BY & 22 & 20 \\
        28 & SUM, WHERE, GROUP BY & 22 & 22 \\
        29 & WHERE, ORDER BY, LIMIT & 8 & 8 \\
        \bottomrule
    \end{tabular}
    \end{table}
    
% \begin{table}
%   \caption{Evaluation of the telemetry results}
%   \label{tab:template_single}
%   %% Footnotesize if a much smaller font is needed
%   %\footnotesize
%   \centering
%   \begin{tabular}{ccccc}
    
%     \toprule
%       colA & colB & colC & colD & colE  \\
%     \midrule
%       %\multirow{3}{*}{\rotatebox{90}{\parbox{1cm}{\centering Image data}}}& \O & 1 in 1,000 & hello  & world  \\
%       FILTER & \O & 1 in 1,000 & hello  & world  \\
%       %FILTER & \O & 1 in 1,000 & hello  & world  \\
%       \multirow{2}{*}{\centering \parbox{3cm}{{FILTER } + {AGGREGATE}}} & \multirow{2}{*}{O} & \multirow{2}{*}{1 in 1,000} & \multirow{2}{*}{hello}  & \multirow{2}{*}{world}  \\  
%        &    &  & &\\
%     One JOIN & \O & 1 in 1,000 & hello  & world  \\  % 
%     Two JOIN & \O & 1 in 1,000 & hello  & world  \\  
%     Three JOIN & \O & 1 in 1,000 & hello  & world  \\ 
%     Three JOIN + AGGREGATE & \O & 1 in 1,000 & hello  & world  \\ 
%     %\midrule

%   % \multirow{3}{*}{\rotatebox{90}{\parbox{1cm}{\centering Table data}}}& \O & 1 in 1,000 & hello  & world  \\
%   %     & \O & 1 in 1,000 & hello  & world  \\
%   %     & \O & 1 in 1,000 & hello  & world  \\
    
%   \bottomrule
% \end{tabular}
% \end{table}

==> EPIC_arXiv/txt/00_abstract.tex <==
\begin{abstract}
    We present EPIC, an AI-driven platform designed to augment operational data analytics. EPIC employs a hierarchical multi-agent architecture where a top-level large language model provides query processing, reasoning and synthesis capabilities. These capabilities orchestrate three specialized low-level agents for information retrieval, descriptive analytics, and predictive analytics. %These agents are integrated with HPC domain knowledge and telemetry data.
    This architecture enables EPIC to perform HPC operational analytics on multi-modal data, including text, images, and tabular formats, dynamically and iteratively.  EPIC addresses the limitations of existing HPC operational analytics  approaches, which rely on static methods that struggle to adapt to evolving analytics tasks and stakeholder demands. 
    
    Through extensive evaluations on the Frontier HPC system, we demonstrate that EPIC effectively handles complex queries. Using descriptive analytics as a use case, fine-tuned smaller models outperform large state-of-the-art foundation models, achieving up to 26\% higher accuracy. Additionally, we achieved 19x savings in LLM operational costs compared to proprietary solutions by employing a hybrid approach that combines large foundational models with fine-tuned local open-weight models.
\end{abstract}


==> EPIC_arXiv/txt/01_intro.tex <==
\section{Introduction}
\label{sec:intro}

%% Opening
Extracting actionable insights from HPC operations has become increasingly important in addressing complex operational challenges rising in the exascale era. 
Operational data analytics (ODA) systems are designed to derive these insights from multi-terabyte data streams originating from modern HPC systems, and play a critical role in optimizing performance, energy usage, reliability, resource utilization, and procurement planning.
Extensive research has been conducted in ODA using telemetry data gathered during HPC operations to study system behavior under various settings and workloads~\cite{netti2019dcdb,netti2020wintermute,patel2020does,shin2021revealing,ott:2020,Bautista:2019,Bourassa2019,shoga2018,wilde20144,icdcs_olcf_24,hpc_workload_trace}. 

%% Shortcoming of state of art
However, the efficacy of conventional ODA techniques is limited when addressing the rapidly evolving needs and increasingly diverse set of stakeholders, as they do not provide dynamic, on-demand, and iterative analytical environments~\cite{NETTI2022102950}. ODA tasks on large datasets are time-consuming and require expertise in data engineering, data science and machine learning. Furthermore, conventional monitoring dashboards offer a static, pre-defined array of visualization charts \cite{dashboard_1, dashboard_2}, further constraining their impact under the on-demand and evolving needs of a diverse stakeholder. 

%% What we present by submitting this paper to the community
The above limitations point to the need for a more flexible, intelligent system capable of adapting to diverse and evolving analysis needs.
To address these limitations and enhance insights derived from HPC operational data, we present the design and implementation of EPIC, an AI-driven platform that leverages the new emerging capabilities of generative AI foundational models \cite{hong2023metagpt, huang2024understanding, zou2024cooperative} into the context of HPC operational analytics. EPIC aims to augment various data driven tasks such as descriptive analytics and predictive analytics by automating the process of reasoning and interacting with high-dimensional multi-modal HPC operational data and synthesizing the results into meaningful insights.

EPIC achieves this goal using a hierarchical multi-agent architecture. This architecture combines generic reasoning and synthesis capabilities of large foundational models with specialized low-level models. These low-level, fine-tuned, open-weight models are integrated into the HPC operational data infrastructure providing access to 1) an unstructured knowledge-base of text, tabular and image data, 2) analytical query into large, structured telemetry data, and 3) seamless interaction with predictive machine learning models trained on past data.
Also, to avoid the high-cost of maintainability and operation of large language models, EPIC leverages a hybrid of powerful proprietary foundational models and local open-source models. As a result, EPIC provides a highly modular yet extensive platform that can easily integrate diverse and heterogeneous operational data analytics capabilities while maintaining cost effectiveness.

%% The summary of our contributions
Our contributions are as follows:
\begin{enumerate}
    %% Contribution 1. It is a new capabiliy...
    \item We design an implementation that demonstrates the role and impact of large language models specialized for HPC operational analytics. The EPIC platform offers on-demand and iterative capabilities, providing a flexible and dynamic interface for exploratory analytics, and is designed to meet the continuously evolving analytical needs. 
    %We present a new capability that can seamlessly automate the multi-modality of HPC operational data with high accuracy which otherwise has been largely human labor intensive. 
    %ahmad
    %\item We developed the EPIC platform to perform ODA tasks by leveraging advanced AI techniques. This platform enables on-demand and iterative capabilities, provides a flexible and dynamic interface for visualization analytics, and is designed to meet the evolving needs of the increasingly diverse stakeholders. 
    %% Contribution 2. We have a novel architecture that enabled this (i.e., we figured out how to integrate GenAI capabilities into our enterprise...
    \item We present a hierarchical multi-agent architecture that facilitates the implementation of cost-effective specialization of generic AI capabilities for HPC operational analytics. EPIC's architecture introduces necessary abstractions to manage the underlying complexities of ODA tasks and provides a user-friendly interactive interface, thereby reducing the need for frequent reliance on data scientists and AI experts.
    %woong
    %\item We present the hierarchical multi-agent architecture that enables us to implement a cost-effective specialization of generic AI capabilities into HPC operations. This architecture provides the necessary abstractions required to modularize major ODA tasks on various modalities of operational data without increasing complexity.
    %ahmad
    %\item This work enhances ODA insights by leveraging the capabilities of multi-agent tools to decompose and synthesize information from diverse and massive datasets, effectively abstracting underlying complexities and thus reducing reliance on data science and AI experts. 
    \item We demonstrate the multifaceted analytical capabilities of the EPIC platform by conducting an extensive evaluation across a diverse range of HPC data-driven queries. We also facilitate the evaluation datasets along with the codebase\footnote{The codebase and data is shared as a part of reproduciblity initiative and AD/AE submission.}.
    %woong
    %\item With extensive evaluation of each of the capabilities, we demonstrate the effectiveness the approaches in EPIC. We explore how the intricate challenges of each data modality can be handled in a cost-effective way and be orchestrated to handle complex descriptive and predictive queries on HPC operational data.
    %ahmad
    %\item Extensive evaluation of models and sharing of corresponding datasets.As our contribution to the ODA research community, we also facilitate EPIC codebase for the researchers\footnote{The codebase and data is shared as a part of reproduciblity initiative and AD/AE submission.}. 
\end{enumerate}

%% The structure of the paper
The rest of the paper is structured as follows: Section~\ref{sec:background} provides a background on current practices in ODA and the applications of LLMs. Section~\ref{sec:design} explains the design and implementation of each component of the EPIC system, including a description of the evaluation pipeline for each module. Section ~\ref{sec:data} presents the EPIC software and the various datasets used in evaluating the models. Section~\ref{sec:evaluation} provides the evaluations of each module and highlights significant findings for each. Finally, Section~\ref{sec:conclusion} concludes the paper.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Backup text below... Will try to reuse it in the background - Woong



%Traditional ODA tasks are typically designed to address predefined queries relevant to specific HPC stakeholders, lacking the flexibility for iterative analysis. 
%Moreover, conventional monitoring dashboards offer a static array of visualization charts, further constraining their impact under the evolving needs of an increasingly diverse set of stakeholders.   

%The impressive cognitive capabilities of LLMs highlight their potential for tasks involving complex processes such as planning, reasoning, and synthesizing optimal solutions. Multi-agent tools, therefore, have the potential to play a significant role in this context~\cite{cheng2024exploringlargelanguagemodel}.

%In one of the DOE office of science articles on HPC research focus areas and opportunity, Office of Science (SC) observed an urgent need for improving the performance of post-exascale HPC system through energy efficiency.
%"\textit{There is a growing consensus that urgent action is needed to address an array of bottlenecks in advanced computing, including energy efficiency...}\cite{doe_sc}". 
%Hardware technologies have contributed significantly in making HPC system energy efficient but with the slowing of Moore's law there is a limited opportunity to further improve the energy efficiency.   

%% Additional details and context - Remove or merge into other paragraphs?
%Emerging ODA challenges highlight the inadequacy of current state-of-the-practice methods. For instance, as emphasized in one of the articles by the DOE Office of Science, 
%"\textit{There is a growing consensus that urgent action is needed to address an array of bottlenecks in advanced computing, including energy efficiency...}\cite{doe_sc}". Given the slowing of Moore's Law, there is limited scope for hardware components to further improve HPC performance~\cite{doe_sc,wes_DT}. Thus, ODA must provide the insights necessary for applications to run optimally, thereby increasing the overall energy efficiency of HPC resources. 


%%% Opportunity to address this problem - Gen AI - Will use this in the background
%AI-driven multi-agent platforms have demonstrated the ability to foster new forms of intelligence to solve complex problems by interaction and synthesizing of information and communicating intermediate results among the various tools\cite{zou2024cooperative}. In particular, Large Language Models (LLMs) have showcased impressive capabilities across diverse domains, exhibiting significant proficiency in reasoning, information processing, tool utilization, planning, and synthesis for various tasks including analytical jobs\cite{hong2023metagpt, huang2024understanding, zou2024cooperative}. In this regard, EPIC platform, leveraging the capabilities of  multi-agent system address the aforementioned limitations of existing ODA techniques. 

%Traditionally, ODA tasks are generally structured to obtain responses to pre-specified inquiries and scenarios pertinent to a particular group of HPC stakeholders~\cite{dashboard_1}.
 %which takes a significant amount of time for end-to-end processing and analytics, and require experts with data science and data engineering backgrounds to accomplish.

%Moreover, different stakeholders have diverse interest in the insights of different aspects of the HPC system. 
%It is frequently challenging to gather requisite information in advance from various data sources and ascertain the most suitable visualization chart and granularity level for a specific group of stakeholders.
%Consequently, we necessitate a platform that is sufficiently adaptable to meet the needs of diverse stakeholders and accommodate changing analytical demands. The analytics platform should mitigate the frequent reliance of various stakeholders on data scientists or engineers for analytics and deliver analytical responses at varying resolution levels to users with diverse backgrounds and interests. 

%In regard to addressing the aforementioned challenges, we have designed and developed EPIC: a large language model (LLM)-driven platform for augmenting HPC ODA tasks. The platform we developed is intelligent enough to reason and guide the query and the response using the agentic framework. The EPIC platform comprises of four modules to address different types of queries, such as descriptive analytics, predictive analytics, or querying information from documents or hybrid queries, which involve more than one tool to respond. The major contributions of the work are as follows:

%\textbf{LLMs-driven, data analytics platform:}
%The LLM-driven dynamic exploratory data analysis platform is designed and developed to respond to questions related to HPC systems without the necessity of frequently building new data analysis pipelines for perpetually evolving analytical requirements. 
%The analytics platform has three main analysis tools or modules: information retrieval analytics, descriptive analytics, and predictive analytics. The analytics platform facilitates tasks such as batch analysis on telemetry data, forecast power, energy and temperature parameters of a future job, and address general-information inquiries of HPC system, components, policies. 
%The platform serves a wide spectrum of HPC stakeholders, which include operations team, engineers, architects, administrators, procurement managers, and executive leadership. In contrast to traditional dashboards, it offers insights and can dynamically provide visualizations at varying levels of detail.

%\textbf{Intelligent reasoning:}
%\textbf{Abstracting complexity with intelligent Query handling and diverse Outputs:}
%In addition to three analytical tools or modules, we also developed top level module to intelligently guide the user queries to the appropriate analytical tool or tools depending on the content and the context of the user's inquiry. The module's ability to intelligently guide queries offers users an abstraction of the underlying complexity, providing responses based on multi-layered reasoning and the synthesis of intermediate responses. The system is also designed to generate the outputs in multiple formats such as standard natural language response, tabular responses, and graphics visualizations of the tabular data.

%\textbf{Extensive evaluation of models, and datasets:} We provide extensive evaluation of the models and also provide the datasets that we used to evaluate the models. Due to the complex nature of the language models and the reasoning and routing modules, we provide evaluations of each tool and a separate integrated evaluation from an end-to-end evaluation perspective. We also evaluate our model with state-of-the-art proprietary LLM models such as OpenAI. We also provide the assessment of the operational cost of the LLM models we incorporated in comparison to the very-large proprietary models.
%We also share the evaluation codes for the future researchers and as a contribution to the HPC research community. 

%\textbf{Facilitating Codebase for HPC operations Community:\footnote{The codebase and data is shared as a part of reproduciblity initiative and AD/AE submission.}}
%As a contribution to the state-of-the-art practice research for the HPC ODA research community, we facilitate the code base of our analytics platform for the research community. We anticipate that this resource, along with the evaluation datasets developed as a part of the state-of-the-art practice research, will significantly help the HPC research team in implementing similar tools at their centers and benchmarking the performance of their tools.



==> EPIC_arXiv/txt/02_background.tex <==
%%
%% e2e framework placed here to make it appear in page 2 upfront
%% Referenced in the design section
%%
\input{figs/framework}
%%

\section{Background and Motivation}
\label{sec:background}
This section outlines the current state of practice efforts in the domain of ODA and the utilization of LLMs and multi-tool agents to enhance analytics. We also demonstrate the applications of LLM and its utilization in various information retrieval and analytical activities.

\textbf{Operational Data Analytics and its challenges:}
Exascale HPC systems, mainly due to the increasing physical footprint caused by the diminishing return in performance per watt in the post-Moore era, the physical side of HPC systems introduces significant challenges such as Power, Energy and Reliability \cite{bergman:2008:exascalecomputing}. While fulfilling the necessary performance, HPC systems need to consider power, energy, cooling, and reliability, balancing many different KPIs all at the same time, thus being exposed to unprecedented cross-cutting complexity \cite{ref:4pillar:2014}.
 
Many HPC sites on the Top500 list are turning towards data as a key resource that can help address the challenges with deploying and operating these large-scale HPC systems \cite{ott:2020}. By establishing a holistic data collection campaign that targets the entire HPC data center, these HPC sites employ powerful data analytics infrastructures that can cope with the 3 Vs of Big Data (velocity, velocity, and variety) seen from these systems.
However, this introduces an inundation of data. Abundance of data enabled such comprehensive ODA infrastructures to introduce new opportunities for innovative data-driven decisions, however, there remain significant challenges in making impact with data. The skill-gap in HPC organizations lacking enough in-house data science expertise introduces bottlenecks in areas such as exploratory data analysis and predictive analysis of datasets \cite{shin:2024-oda}. 

The EPIC analytics platform can reduce this gap by facilitating HPC ODA tasks for users with varying degrees of data science expertise, thereby diminishing reliance on data science specialists.

\textbf{Current practices: Descriptive and Predictive Analytics:}
Netti et. al. \cite{netti2021} introduces a conceptual framework for HPC operational data analytics that can be applied to distinguish different capabilities of data analytics seen in HPC centers. The framework maps descriptive \& diagnostic (hindsight), and predictive \& prescriptive (foresight) data analytics \cite{lepenioti2020prescriptive} use cases in operational domains spanning across four different pillars~\cite{ref:4pillar:2014}.

In practice, the most frequent hindsight-driven analytics is descriptive, manifested in capabilities such as dashboards and interactive visualizations that can answer the question of “what happened?” \cite{ott:2020}. 
Also, in foresight, use cases in predictive analytics are frequently explored, reflecting the excitements in the potential of more advanced data science techniques manifesting in the form of various machine learning models trained from past data and being deployed to make predictions of future system behavior~\cite{sukhija_towards_2022, molan_semi-supervised_2022, shoukourian_forecasting_2020, bartolini_paving_2019} that can enhance existing dashboards or visual analytics systems.

However, such use cases suffer from the rigidity of these dashboards or analytics services both consuming long-development cycles \cite{shin:2024-oda} and being quite fixed to a certain use-case or a scenario~\cite{dashboard_1}. 
%It is difficult to keep up with the needs of an HPC site, especially in a dynamic environment where the questions being asked can evolve. This motivates us to think of more flexible ways of interacting with operational data.
Meeting the analytics requirements of an HPC site is challenging because of continuously evolving inquiries. This inspired us to develop EPIC to incorporate dynamic, interactive methods for engaging with operational data to do exploratory data analytics and derive insights. 

\textbf{Applications of Large Language Models:}
Large Language Models (LLMs) have showcased impressive capabilities across diverse domains, exhibiting significant proficiency in reasoning, information processing, tool utilization, planning, and synthesis for various tasks including analytical jobs~\cite{hong2023metagpt, huang2024understanding, zou2024cooperative}. AI-driven multi-agent platforms further extend these capabilities by enabling collaboration among specialized agents that can interact, synthesize information and share intermediate results to solve complex problems\cite{zou2024cooperative}. 

In high-performance computing (HPC) and scientific research, open LLMs such as LLaMA series \cite{touvron2023llama}, Falcon \cite{almazrouei2023falcon}, Mistral \cite{jiang2023mistral}, BLOOM \cite{bigscience2022bloom}, etc. have been applied to automate code generation \cite{ValeroLara2023ComparingLA, kadosh2023scope}, parallelization \cite{10.1007/s10766-024-00778-9}, and workload orchestration \cite{Kadosh2023MonoCoderDC}.
%While general-purpose models like GPT-3 \cite{} and LLaMA perform adequately for serial code, they often fail to produce performant parallel HPC code (e.g., OpenMP, MPI), highlighting a gap in domain specificity. This has led to the development of HPC-adapted models like HPC-GPT \cite{} and MonoCoder \cite{}, which outperform larger general models by being trained specifically on C/C++/Fortran scientific workloads—successfully detecting data races and suggesting optimizations for parallel execution \cite{}\cite{}.
%Moreover, LLM agents integrated with tools like LangChain \cite{} and Parsl \cite{} have shown real-world success in orchestrating simulations on supercomputers (e.g., Polaris HPC system), where researchers can initiate molecular dynamics simulations through natural language prompts, bypassing the complexities of job schedulers \cite{}).
Frameworks such as HyCE \cite{Miyashita2024LLMAH} further enhance LLM utility by grounding responses in real-time cluster state, improving the safety and reliability of LLM-driven system interactions in HPC environments.
Similarily, chatHPC \cite{Yin2024chatHPCEH} based on FORGE \cite{Yin2023FORGEPO} is another application of LLMs for High-Performance Computing knowledge discovery and question answering.

%In cloud computing and energy-aware scientific applications, open LLMs are leveraged for large-scale distributed simulations, intelligent resource scheduling, and AI-as-a-service deployment. A real-world case by AWS uses LLaMA-based agents in a Ray-ParallelCluster setup to model an AI-driven energy market simulation, capturing emergent dynamics of distributed supply chains—an approach that allows adaptive agent behavior in scientific policy modeling \cite{}. 
%Simultaneously, projects like NASA and IBM’s INDUS trained open-domain LLMs for climate science and deployed them via cloud platforms for broad accessibility in Earth system research \cite{}. 

%In terms of energy efficiency, LLMs have shown promise in refactoring scientific code to reduce energy usage—improving runtime power consumption by up to two times compared to traditional compiler optimizations \cite{Peng2024LargeLM}. 
In system monitoring, LLMs fine-tuned with system logs and observability data are being applied to summarize HPC/cloud system failures \cite{10.1145/3643916.3644408}, detect anomalies \cite{Egersdoerfer2023EarlyEO}, and even suggest mitigation strategies \cite{Qi2023LogGPTEC}, laying the groundwork for self-healing infrastructure in scientific computing environments. All these works underscore how open LLMs are revolutionizing scientific computing by enhancing operational intelligence, energy-aware scheduling, and user accessibility across both HPC and cloud platforms.

Inspired by these advances, we are motivated to explore the application of LLMs in the context of HPC operational data analytics. We envision the EPIC platform assisting its users in navigating and analyzing heterogeneous HPC operational data, thereby solving the "last-mile problem" in ODA.


==> EPIC_arXiv/txt/03_design.tex <==
\section{EPIC Design and Implementation}
\label{sec:design}
In this section, we begin with a high-level, end-to-end description of the EPIC architecture. Subsequently, we delve into the design of each module. Then we present the design of the evaluation pipeline.

\subsection{Architecture}
\label{subsec:architecture}
 Figure~\ref{figs:architecture} illustrates the architecture of the system. Here, we primarily address the integration of 
 %LLMs into a HPC operational data analytics infrastructure by 1) identifying what LLMs are capable of and 2) by employing the necessary structures to control the complexity and its impact to the rest of the system.
 analytical tools driven by LLMs into HPC operational data analytics infrastructure by 1) identifying which LLMs work best for accuracy, efficiency, and performance and 2) by employing the right structures for workflow orchestration and develop a complex and dynamic \texttt{Query Processing Module}  and \texttt{top-level} model for navigating the users queries and its impact on the rest of the system.
\subsubsection{Framework}
\label{subsec:architecture:framework}
With the data and model access layer (Fig.~\ref{figs:architecture}-a) and the hierarchical LLM interaction layer (Fig.~\ref{figs:architecture}-b), the architecture provides a composable way to 
accommodate various low-level capabilities of HPC operational data analytics into a single intelligent system. Each low-level capability tool
%corresponds to the access to the influx of various ingest 
involves accessing the influx of various data inputs from the HPC operational environment (Fig.~\ref{figs:architecture}-a). Such capabilities include the retrieval of domain knowledge and interactions with the telemetry database and predictive models, which are then exposed to the LLM interaction layer.

The LLM interaction layer (Fig.~\ref{figs:architecture}-b) is responsible for bridging the gap between natural language ongoing conversation with human operators and underlying data and tools or agents. Architected in a hierarchical fashion, the user interaction, represented as the message history is broken down into subtasks by a top-level Query Processing (QP) Module. These sub-tasks are then “delegated” to lower-level agent(s) and tool(s) based on the content and the context. The sub-tasks are then executed, and their results are recorded back into the message history. 
The QP module will then synthesize the results to respond to the original user query(Fig.~\ref{figs:architecture}-c). 
With this hierarchical architecture,  we have added three modules at the lower level: the \textit{Information Retrieval (IR)} Module, the \textit{Descriptive Analytics (DA)} Module, and the \textit{Predictive Analytics (PA)} Module (Fig.~\ref{figs:architecture}-b). The system can be easily extended by adding more instances at the lower-level without affecting existing lower-level agents or top-level QP module. 
%of ingest pipeline and exposing the new types of system state to a low-level LLM in the LLM interaction layer without introducing significant changes to the other capabilities. 
The design provides users with an abstraction layer, enabling them to perform a wide range of on-demand, iterative analytics, including complex multimodal tasks,
%from one or more underlying models 
without worrying about the complexity.
\subsubsection{Hierarchical Agentic Query Processing Module}
\label{subsec:architecture:agentic_routing}
At the core, this architecture leverages LLM driven agentic query processing and tool calling loops designed to perform specific tasks depending on its role, level, and capabilities given (Fig.~\ref{figs:architecture}-b). Leveraging the reasoning, planning, tool calling, and information synthesizing capabilities, the QP module provides an autonomous recursive interaction between itself and the lower-level agents. This provides the system with a capability 1) to reason about how to coordinate the interaction with the environment and 2) recover from errors if any happened. We have found this capability crucial to bridge the gap between the non-determinism inherent in these LLMs and the determinism that the rest of the system requires.

Further, the “tool calling” capability enables hierarchical design that promotes composability. Instead of a monolithic interaction between the human operator and the underlying environment, the LLM interaction layer is divided into a top-level manager agentic loop for orchestrating delegations and several low-level agentic loops for specific data interactions as shown in boxes in Fig.~\ref{figs:architecture}-b). 
This hierarchical and modular design also enables the \textit{QP} module to respond to complex queries that necessitate interactions with multiple modules. For instance, to determine the number of HPC jobs utilizing GPUs, the \textit{IR} module must first supply the domain information regarding idle power. Subsequently, the \textit{DA} module can filter jobs in the telemetry data that exhibit GPU utilization exceeding this idle power threshold. 
The \textit{QP} module routes the user question to first \textit{IR} and then \textit{DA} agents and then synthesizes the intermediate results from  these modules to finally respond to the user question.



%We have it in 3.1.1
%Whenever a new capability is introduced, this system is extended by implementing a new low-level ingest pipeline and a dedicated low-level agentic tool-calling loop to ensure a reliable interaction. This agentic loop is then integrated into the top-level module as another tool without any changes to its structure.
 
  \subsubsection{Information Retrieval Module} %Docs
  The Information Retrieval (\textit{IR}) module or agent in the EPIC system is handles HPC-specific queries and retrieves relevant domain information from HPC user manuala, web, academic papers, HPC's auxiliary systems manual. 
  In addition to text responses, the \textit{IR} module also provides structured data in the form of tables and graphical information as images. 
  The \textit{IR} data ingestion pipeline shown in Figure~\ref{figs: document_module} consists of several tasks: chunking, semantic retrieval with hash-based indexing for tables, a reranker for candidate selection, and the \texttt{Llama-3.1-8B} large language model for final response generation. This integrated approach enhances user interaction by returning rich, contextually accurate responses that include both textual and visual data. 
  %Figure \ref{figs: document_module} is a schematic of our \texttt{IR} module. We implement the document module retrieval-augmented generation (RAG) pipeline using the LangChain \cite{langchain} framework.

 The \textit{IR} retrieval-augmented generation (RAG) system architecture comprises five integrated sub-modules that transform user queries into contextually relevant responses from HPC documentations. The \textit{IR} module has its own \textit{Query Interpretation (QI)} sub-module that performs decomposition of complex queries into sub-queries and expands wthem with domain-specific terminology. The \textit{IR} module handles content chunking based on semantic coherence and specializes in \textit{multimodal content processing}, extracting tables and images from HPC documents.  
 %and generating descriptive textual representations via an LLM (\texttt{GPT-4o} here) to enable semantic retrieval of these non-textual elements. 
 During the pipeline building phase, the tables from the HPC documentation re processed using \textit{GPT-4o} to generate their descriptive textual representations. These descriptions capture the semantic content and purpose of each table, enabling retrieval based on the information they contain instead of only their surface structure.  For image data, embedded images are extracted using \textit{openai/clip-vit-base-patch32} model, and their captions and additional text is generated with \textit{GPT-4o}. This ensures that diagrams, charts, and other visual elements in the documentation become retrievable during inference phase. 
 The \textit{IR} module leverages ChromaDB as a vector database, employing hybrid retrieval techniques that combine dense vector similarity matching (\textit{mxbai-embed-large-v1}) with sparse retrieval and filtering capabilities. Separate vector databases store table and image embeddings along with their textual descriptors using \textit{Mixed-Bread} \cite{emb2024mxbai} general-purpose light-weight embeddings (512 dimensions). 
 The retrieved content undergoes refinement in the \textit{Re-ranking} sub-module (\texttt{mxbai-rerank-large-v1}), which scores chunks based on semantic relevance, content authority, and information freshness while promoting diversity in results to ensure comprehensive coverage of decomposed queries. This sophisticated inference pipeline ensures that textual content, tables, and embedded images are all accessible through semantic querying. 
 The \textit{Generation} sub-module synthesize coherent responses by integrating retrieved content chunks into an optimized prompt structure. The module's design enables it to seamlessly incorporate information from text, tables, and images into unified responses that directly address user queries about HPC documentation.  
    \input{figs/design_document_module}
    
    \subsubsection{Descriptive Analytics (\textit{DA}) Module} %SQL
    %\ahmad
    %The ODA tasks, such as descriptive analytics on the retrospective datasets, are the focus of the descriptive analytics (\texit{DA}) module's design. 
    The \textit{DA} module is designed to facilitate users from diverse backgrounds in performing iterative, exploratory ODA tasks on retrospective telemetry data. 
    Figure~\ref{fig:telemetry_module_diagram} illustrates the various components and the workflow of the DA module pipeline. 

    Whenever a user query is delegated to the DA module, it is concatenated with instructions and schema information. Instructions provide the context to the model, helping it understand the query better and respond effectively. The schema information includes descriptions of telemetry data stored in tables, such as table names, field names, and relationship between tables. The combined input is then processed by the fine-tuned open-weight \texttt{Meta-Llama-3-8B-} \texttt{Instruct} LLM model~\cite{defog_sqlcoder}. The model generates a SQL for the input prompt. The agentic-reflection loop validates the generated SQL for syntax and schema. If the validation fails the model revises the generated SQL, and the process repeats until a valid SQL query is generated or a maximum number of retries is reached. The final SQL query is then executed on the database, providing the response to the analytical query. The user interface, introduced later, offers on-demand interactive graphical visualizations to illustrate the datasets. 
 
    %To address this evolving nature of the analytics requirements, and to reduce the frequent dependency on data scientists, we incorporated the LLM models to build the DA module. The LLM model we used is finetuned for structured query language (SQL) for database on the top of base \texttt{Meta-Llama-3-8B-Instruct} model. The model translates the diverse range of natural language questions into SQL, which helps in exploratory data analysis tasks. 
    
     \input{figs/design_telemetry_module}

    \subsubsection{Predictive Analytics (\textit{PA}) Module} %SQL
     %\naw     
     The PA module is designed to handle tasks that estimate HPC job metrics, such as power utilization, energy consumption, and compute node temperature. Figure~\ref{figs:prediction_diagram} illustrates the components and workflow of the prediction module, which consists of two sub-modules.
     %We use this module for predictive analysis to help users with predictive questions relevant to power, energy, and temperature data of Frontier supercomputer based on a year of Frontier historical data that we used to train a deep neural network-based regression model. 
     %The components and workflow for the prediction module is given in Figure \ref{figs:prediction_diagram}. The overall module is divided into two sub-modules. 
     
     The first sub-module  is the \textit{Query-Interpretation (QI)}, which interprets user questions directed by the top-level \textit{QP} module to the \textit{PA} module. Similar to the \textit{DA} module, the \textit{QI} agent uses the \texttt{Meta-Llama-3-8B-Instruct} model, fine-tuned for translating natural-language into structured format. 
     Before processing the query, it is combined with information such as science domain names, their descriptions, feature names, and descriptions to assist the model in interpreting the questions correctly. This model then converts the input queries into a structured format, identifying the input and output variables needed for the regression models to estimate the output value. 
     If users do not provide all input features, the model handles this by using a set of the most frequent values for the missing inputs.
     %This model translates input queries into a structured format, identifying the input and output variables required for the regression models to estimate the output value. %The input and output variables returned by \texttt{query-interpretation} submodule is generated as the structured `json' format. We use the base \texttt{Meta-Llama-3-8B-Instruct} model and finetune it for translating the user questions into a set of input values, and output feature(s). 
     %We combine the query with the informations such as science domain names, their description, the feature names and their descriptions in the input prompt to assist the model to interpret the questions correctly. 
     %Regression models always require a fixed number of input variables, and in case the users do not provide some of the input features in their question, we handle this by providing a set of most frequent values for the missing input features. 
     %All the question-answer pairs are human evaluated because multiple answers can be accepted for the same question.  The LLM might return a variation of the answer that is also correct. If the LLMs fail to deliver exactly correct structured output format, the post-processing script converts the LLM output into correct json format.
     %Based on the input feature values, and the output feature(s) received from the LLM response, the prediction is done using the regression model feeding that LLM output. 

     The second sub-module employs regression models, including a feedforward neural network and a regression decision tree, to perform prediction tasks. For instance, the PA module can address queries such as, \textit{"Estimate the total amount of energy consumed by a job that runs on 1,000 compute-nodes, belongs to the computational fluid science domain, and runs for 2 hours."} These regression models are designed to predict one of the 16 features related to power, energy, and temperature, as detailed in Table~\ref{tab:prediction_feature_summary}. The input features include the science domain, walltime, number of nodes, and whether the job utilizes CPU or GPU. A combination of regression models is employed because neural network models provide better accuracy for certain output features, while regression decision tree models outperform neural networks for others. The prediction results are then returned to the top-level model for synthesis and redirection to the user interface for rendering.
     %The second submodule contains regression models(feedforward neural network model and regression decision tree model) to accomplish prediction tasks. In particular, our \textit{PA} module answer questions such as, "Estimate total amount of energy consumed by a job that runs on 1000 compute-nodes and belong to comuptational fluid science domain and runs for 2 hours."
     %The input values and the output variable of the prediction model can be easily parsed from the structured json generated above. 
     %For the regression task, we designed and implemented a feedforward neural network using the PyTorch framework. The core of the model consists of three hidden layers followed by an output layer. 
     %We use 13 months of historical data to train our model. 
     %The regression models are designed to predict one of the 16 features related to power, energy, and temperature given in Table \ref{tab:prediction_feature_summary}. The input features set contains science domain, the walltime, number of nodes, and whether the job utilizes CPU or GPU. We are using combination of regression models because for some out features neural-network models gives better accuracy whereas, for some other features simple regression decision tree model outperforms neural-network model. The prediction results are returned back to top-level model for it to synthesize and redirect it to the user interface for rendering. 
     
     %Besides, the deep learning-based model, we also experiment with traditional regression models to see the performance differences. We find that particularly for the energy-based features the decision tree (DT) model has lower errors. So, for the energy features we use the DT model. As the number of features might increase depending on data availability, decision trees can become computationally expensive and less effective compared to the Deep Neural Networks (DNN). So, we prefer the DNN model for better generalization capabilities for the rest of the Power and Temperature features. In Section \ref{sec:evaluation}, we report our regression results accordingly.  



\input{figs/design_prediction_module}

\input{tables/prediction_output_feature}

  \subsubsection{Multi-modal Rendering User Interface}
    %\jesse
    
    Users interact with the EPIC system via a chat bot style web UI. The user can prompt the model and get text responses, tables, and/or plots in response. Using the agentic routing, the UI allows the user to interact with the \textit{IR}, \textit{DA}, and \textit{PA} modules as needed based on their query.
    %If a user prompt requires querying the descriptive analytics module and/or predictive analytics module to answer, the module results will be displayed as a table, a figure, and a plot. 
    Unlike conventional chat bots, we chose to make the web UI output plots as dynamic widgets. Users can interact with the widgets to change the plot type and data columns rendered, e.g. to switch between line and bar charts, or to select a specific portion of the data which is relevant. This flexiblity allows users to easily customize the plot rendering to fit their specific use case.
     
    We wanted to avoid the AI agent being a "black box", and to allow users to inspect the agent's reasoning process. The UI displays intermediate steps and tool calls the agent makes in expandable sections in the chat. In addition, if the user prompt requires querying the \textit{DA} module to answer, the generated SQL can be shown in a side window along with the tables and plots, at the user's discretion.
  
\subsection{Evaluation Pipeline}
    %\ahmad~
    Evaluating the EPIC system is essential for assessing its quality and fostering confidence in its wide-ranging, multifaceted HPC operational analytics capabilities. We present an extensive analysis of the \textit{IR}, \textit{DA}, and \textit{PA} modules, along with an evaluation of the top-level Query Processing Module. This includes an end-to-end assessment to demonstrate combined performance on hybrid questions that require multiple tool calls. We detail the extensive evaluation results in Sec.~\ref{sec:evaluation}.  
    %The evaluation of the EPIC system is crucial for assessing its quality and fostering confidence in the EPIC platform. We present a extensive analysis of all three modules---the \texttt{IR} module, the \texttt{DA} module, and the \texttt{PA} module—individually, along with an evaluation of the top-level \texttt{Query Processing Module} which evaluates EPIC's agentic reasoning, routing, and synthesis capabilities. It also provide an end-to-end evaluation to demonstrate their combined performance on hybrid questions---those questions that require the use of more than one tool within the EPIC platform. 
    
    %\woong~
    \textit{High-level Reasoning, Routing, and Synthesis Evaluation~} 
    We evaluate the top-level hierarchical routing described in Sec.~\ref{subsec:architecture:framework}, a critical element for composability and extensibility. 
    Our assessment focuses on whether the model can accurately "route(delegate)" user requests to the correct low-level agents and synthesize the results. We report metrics including routing accuracy, synthesis accuracy, and total token cost. 
    %We evaluate the capability the hierarchical routing primarily described in Sec.~\ref{subsec:architecture:framework} which is a critical element that enables composability and extensibility while minimizing complexity. Handled by the higher-level model and its agentic tool calling loop, we evaluate whether the high-level model can “route (delegate)” the user request to the correct low-level capability by reasoning about when and in what order. While doing so, we ensure the result of such delegations are well synthesized and accurately presented back as a response. In our evaluations, we report routing accuracy, synthesis accuracy, and total token cost.

    \textit{Information Retrieval Module Evaluation: }
    Evaluation of the multi-modal Retrieval Augmented Generation (RAG) system ensures robust and contextually relevant retrieval and generation of HPC knowledge-base and documentations; please refer to Section 5.1 for details. %Our textual evaluation employs automated NLP metrics (ROUGE, BARTScore, BERTScore), human evaluation for relevance and accuracy, and LLM-as-judge offers scalable, consistent validation. For multimodal retrieval, we use Top-1 Accuracy and Mean Average Precision (MAP) to quantify the system’s efficacy in retrieving tables and images.
    %Comprehensive evaluation of the multimodal Retrieval Augmented Generation (RAG) system is essential for ensuring robust, accurate, and contextually relevant retrieval and generation of both textual and multimodal HPC documentation. Given the critical importance of precision and reliability in HPC environments, our textual evaluation employs a multi-layered approach: automated NLP metrics (ROUGE, BARTScore, BERTScore) quantify linguistic quality; human evaluation ensures relevance, coherence, factual accuracy, and completeness aligned with domain expertise; and LLM-as-judge assessments offer scalable, consistent validation. This triangulation overcomes individual method limitations, delivering thorough confidence in the generated textual outputs.
    %
    %Moreover, rigorous evaluation of multimodal retrieval—particularly tables and images—is vital to address the unique challenge of accessing complex information embedded in visual and structured forms frequently found in HPC documentation. By leveraging established information retrieval metrics such as Top-1 Accuracy and Mean Average Precision (MAP), we quantify the system’s efficacy in accurately retrieving multimodal content based on textual descriptions and captions. Such comprehensive assessment not only ensures reliability across diverse content types but also directly aligns with HPC practitioners’ needs for precise, integrated insights into operational analytics.
     
     %\ahmad~
     \textit{Descriptive Analytics Module Evaluation:~} 
     %The primary task of the DA module is to perform operational analytics on user queries. 
     We evaluate the \textit{DA} agent by comparing the datasets extracted from generated SQL queries against the datasets generated by gold-standard queries. 
     This approach is selected because multiple correct SQL statements can produce the same dataset, as illustrated by queries (a) and (b) in Figure~\ref{fig:telemetry_module_diagram}.
    
    However, evaluating datasets rather than SQL statements presents several challenges. Column names may differ between datasets even if the data is identical. Additionally, the order of data rows can vary, which is important for tasks like retrieving the top k rows. Furthermore, datasets may have matching values but differ in row-to-row mapping. 
    To address these challenges, we mark a response as correct only when the data in the columns matches the data generated by the gold-standard queries, regardless of column names, and when the row order and mapping are accurate.
     %The \texttt{DA} module main task is to analyze the historical data based on the questions asked. Thus, for the \texttt{DA} module, we perform the evaluation of the LLM models based on how accurate the extracted dataset for a query compared to ground-truth dataset. For every question, we compare the dataset extracted from the SQL query, which was generated by the LLM model, with respect to data generated from the ground truth queries. 
     %The evaluation metric we used is the accuracy of the model; by which if the two datasets match we evaluate it to 1 and if it false we evalute it to 0. For the evaluation we try to classify 

    %We evaluate the datasets generated from the SQL query and not the SQL statements themselves because at times there could be more than one correct SQL statement to generate exactly the same dataset (as shown by two queries in Figure~\ref{fig:telemetry_module_diagram}). 

     %However, comparing two datasets is also non-trivial and presents several challenges. When we compare the two datasets, it is possible for the column names in each dataset to differ, even though the columns in the two tables may contain exactly the same data (refer to the column names in the two SQL statements in Figure~\ref{fig:telemetry_module_diagram}).  For evaluation, we mark the response as correct only when the data in columns match with the data generated from ground-truth queries and not only the name of the columns. Another issue is that, even if the datasets generated from the two SQL queries are identical, their order may differ, potentially leading to incorrect conclusions, particularly when the order of the data is significant, such as in the case of the top \texttt{k} rows. Finally, the third issue is that the two datasets could have matching values for all columns, but the one-to-one mapping of each row in the dataset may not align. We show the extensive evaluation results in Sec.~\ref{sec:evaluation}.

    %\input{EPIC/figs/sql_comparision}
     %\naw~
     \textit{Predictive Analytics Module Evaluation:~}
     The \texttt{PA} module comprises two main components: the \texttt{query interpretation} sub-module and the \texttt{regression} module. For query interpretation, we use the accuracy metric to assess how well the model converts user input into structured JSON. Specifically, we evaluate the accuracy of each of the four input features and the output feature, which can be any one of the 16 features (refer to Figure 1). For evaluating the prediction regression sub-module, we employ three error metrics to assess the model's performance: Mean Absolute Error (MAE), Root Mean Square Error (RMSE), and Mean Absolute Percentage Error (MAPE).
     %The two main components of the \texttt{PA} module are the \texttt{query interpretation} submodule and the \texttt{regression} module. For query interpretation, we use the accuracy metric to calculate how well the model is able to convert the user's input to structured 'json.'
     %For the evaluation of the prediction regression submodule, we use three different error metrics to learn about the model's performance. We use: Mean Absolute Error (MAE), Root Mean Square Error (RMSE), and Mean Absolute Percentage Error (MAPE) to report the models' performance. 
     

==> EPIC_arXiv/txt/04_data.tex <==
\section{EPIC Software \& Data}
\label{sec:data}
    In this section we describe the EPIC platform software and datasets that we used for evaluating the various modules.
    \input{tables/models_and_data}
    %The core of our evaluation focuses on the performance of the hierarchical LLM interaction layer.  
    %The top level consists of a custom agentic loop, which uses LLM tool-calling to invoke the lower-level modules. 
    The top-level \textit{QP} module consist of agentic loop to call lower-level agents. 
    Each of the modules are implemented using LangChain v0.3~\cite{langchain}.  
    The \textit{IR} module stores documents in ChromaDB v0.6~\cite{chromadb}, the \textit{DA} module's telemetry database uses the library based (DuckDB v1.1~\cite{duckdb}), and the regression models are trained using Pytorch v2.6~\cite{pytorch}.  All the components are integrated together in a Chainlit v2.2~\cite{chainlit} based chat UI.  
    Data for each access point is ingested into the system via out-of-band pipelines, separate from the hierarchical LLM interaction layer, (see Figure~\ref{figs:architecture}).

    Due to the varied natural language capabilities, each component leverages different underlying LLMs. 
    This resulted in a several Llama~3 based fine-tuned models \cite{grattafiori2024llama3herdmodels} for low-level components and OpenAI models \cite{openai2024gpt4ocard} for the high-level reasoning, routing, and synthesis.

    The EPIC design allow each component can be imported separately from an out-of-band evaluation pipeline, enabling batch end-to-end tests without the WebUI. With the data already ingested, the code-paths for each component in the LLM interaction layer has been evaluated as if deployed in a real environment. 
    %With such preparation, we evaluated 1) the \texit{IR} module, 2) the \texit{DA} component, 3) \texit{PA} model separately, and 4) the top-level \texit{Query Processing Module} having reasoning, routing, and synthesis module independently leveraging the datasets specifically prepared for each component.

    Table~\ref{tab:models_data}, summarizes the dataset prepared for evaluating all components of the EPIC platform. 
    For evaluating \textit{IR} module, we curated a \textit{gold-standard} set of Q\&A pairs, written by subject-matter experts to simulate real HPC center queries. The Q\&A pairs include textual data, as well as tables and images from documentations. 
    %The subject-matter experts wrote \textit{relevant} question and answers simulating real queries from OLCF users. The question-answer pairs were not just textual, but also include tables and images from the documentations. 
    %We use this dataset as our evaluation dataset currently which is a mix of text-only, table-based, and image-based Q\&A pairs. %However, we plan to fine-tune our underlying LLM on the ``enhanced" version of this dataset to facilitate better "multimodal question-answering" in the future.
     
    %\ahmad~
    %In Table~\ref{tab:models_data}~we show summary of the dataset used for evaluation of different component of the EPIC's ODA platform. 
    The \textit{DA} evaluation dataset contains about 500 natural language questions and SQL response pairs. We also maintain a generated telemetry dataset schema for performing analytics on energy, power, temperature and their corresponding scheduler logs. 
    %As already mentioned in the earlier section, we do not compare the SQL directly rather we compare the datasets extracted from the database using the generated queries and the ground-truth queries.
    The schema definition data, including table names, column descriptions, data types, and table relations is important part of the input prompt alongside natural language questions.

    The~\textit{QI} sub-module of the Predictive Analytics module evaluation dataset includes 100 prediction Q\&A pairs related to power, temperature, and energy consumption of supercomputer jobs. The ground-truth responses are structured in JSON format. For the regression sub-module, we used 80\% of one year's worth of $0.5$ million Frontier job-level data for training and 20\% for evaluation.
    %The ~\textit{QI} sub-module of the Predictive Analytics module evaluation dataset includes 100 prediction Q\&A pairs. 
    %related to power, temperature and energy consumption of supercomputer jobs. The ground-truth responses are structured in 'json' format.
    %output that is translated and extracted from the user question, and readily available to feed to the prediction regression model.  %and  that covers all of the Table~\ref{tab:models_data}~b~
    %For the regression sub-module, we used 80\% of one-year of 1.1 million Frontier job-level data for training and 20\% for evaluation.
    %we have $20\%$ of the Frontier Job-level Power data separated as Test Set for evaluating the performance of the regression model.

==> EPIC_arXiv/txt/05_evaluation.tex <==
\section{
    Empirical Evaluation }
    \label{sec:evaluation}
    %\ahmad~
        Using the application software and data, we conducted extensive quantitative evaluations of each module, including top-level end-to-end evaluations for synthesis and routing. The LLM models across different modules have varying inputs and outputs, leading to distinct metric criteria. These criteria validate various aspects of the EPIC modules.
        %\subsection{Descriptive Analytics}
        \input{tables/document_RAG_text}
        \subsection{Information Retrieval Module} Our Information Retrieval module is a Retrieval Augmented Generation (RAG) system for HPC-centric question-answering. The responses from this multimodal module is critical for user-queries on HPC documentation and knowledge.
    
        ~\textit{Lexical and Semantic evaluation}: We employ standard Natural Language Processing (NLP) metrics to evaluate the answers generated by the \textit{IR} module.
        To capture both lexical and semantic essence, we use ROUGE metrics \cite{lin-hovy-2003-automatic} for lexical and BERTScore \cite{DBLP:conf/iclr/ZhangKWWA20}; BARTScore \cite{10.5555/3540261.3542349} for semantic similarity with ground-truth data. 
        The objective is to assess how well our generated answers reflect the actual answers for the given queries at both lexical and semantic levels.
        %ROUGE scores are commonly used for evaluating generated answers in QA, especially for extractive responses. ROUGE-1 measures unigram overlap, capturing basic content similarity. ROUGE-2 focuses on bigram overlap, reflecting fluency and phrase-level coherence. ROUGE-L measures the longest common subsequence, emphasizing structural similarity. While useful, ROUGE can miss semantic correctness, so it is often paired with metrics like BERTScore or human evaluation, which we do further.
        For lexical evaluation (Table \ref{tab:doceval}), we use ROUGE-1 and ROUGE-L, as fluency and coherence (ROUGE-2) are captured in our human and LLM-as-judge evaluations.
        %Table \ref{tab:doceval} shows our performance. 
        The lexical evaluation (via ROUGE scores; ROUGE1 and ROUGE-L) reveals that the system has a performance-affinity towards generating concise answers withhigh precision but low recall, effectively avoiding noise but sometimes misses relevant content.
        
        However, lexical metrics do not capture semantic similarity (paraphrases, synonyms) and can penalize valid answers if phrasing differs, and can be gamed by long answers with keyword stuffing. 
        Hence, we perform semantic-level evaluation of our system-generated answers against gold-standard. 
        BERTScore is a semantic-level Natural Language Generation (NLG) evaluation metric based on token-level Precision, Recall, and F1, utilizing contextual embeddings from the BERT language model \cite{devlin-etal-2019-bert}. It compares predicted and reference texts using contextual embeddings, capturing meaning beyond exact word overlap. This make BERTScore well-suited for evaluating paraphrased or abstractive QA answers. From Table \ref{tab:doceval}, BERTScore-F1 is 0.62 which is considered to be \textit{good} with some paraphrasing or minor errors. 
        However, like the lexical metrics we observe high precision and low recall situation. This signifies that our generated answers are concise, and hence may not be adequate enough in some cases.
 
        We also employ BARTScore, a semantic evaluation metric inspired by text-generation model BART \cite{lewis-etal-2020-bart}, commonly used for longform QA evaluation. 
        BART score measures the 
        %BARTScore is a learned evaluation metric using the BART model that measures the 
        likelihood of reference text given the generated text providing a more semantically aware than ROUGE or BLEU. However, BARTScore values are negative log-likelihoods, so less negative indicate better performance. 
        From {Table \ref{tab:doceval}, BARTScore-F1 is -4.12 which, while not ideal, reflect the concise nature of generated answers. 
        This score suggest, generated answers is likely relevant and partially correct, but may be missing details, consistent with the lexical evaluation.}
        
        One critical issue with Generative AI models is \textit{Hallucination}, where generated answers sound plausible but contain incorrect information. 
        Lexical and semantic NLG metrics do not verify factual correctness, only linguistic similarity. 
        %As a result, a generated answer can sound plausible and score well while containing unsupported or incorrect information. 
        To address this, we combine these metrics with faithfulness checks, such as entailment models or human judgment. 
        We use the SelfCheckGPT-NLI \cite{manakul-etal-2023-selfcheckgpt}, an automated Natural Language Inference (NLI)-based metric for hallucination evaluation.
        SelfCheckGPT-NLI detects hallucinations by measuring contradictions between generated answers and multiple sampled outputs.
        A higher contradiction score indicates lower factual consistency. 
        A SelfCheckGPT-NLI score of 0.45 signifies a moderate-low likelihood of hallucination in the QA answer.
        
        \textit{Multimodal Information Retrieval: }We evaluate the multimodal information retrieval capability of the \textit{IR} module in Table \ref{tab:table-image-retrieval}, using metrics like Top-k (k=1) Accuracy and Mean Average Precision (MAP).
        These metrics asses whethercorrect images and tables are retrieved. 
        We penalize responses that generate only text-based answers for multimodal questions. 
        The Top-1 accuracy metric is `strict/hard match' and a score of 0.68 for image and 0.65 for table, indicating good performance. 
        MAP scores (lenient than Top-1) are based on retrieval @ 2 (see Table \ref{tab:table-image-retrieval}) indicates precise retrieval of relevant construct (table/image) in response to user queries.
        %\tirthankar~
        
        \textit{Human Evaluation and LLM-as-judge}: Automated NLP metrics are still not adequate to cover the full spectrum of evaluation. 
        Hence, we employ \textit{human evaluation} using criteria such as \textit{Correctness, Completeness, Fluency, Relevance} on a Likert scale of 1-5. Table \ref{tab:human-llm-eval}.
        An HPC domain expert rated the generated answers, finding them highly coherent and relevant, with strong-alignment to input queries. Relative lower factual accuracy indicate occasional inconsistencies, Completeness core indicate reasonable coverage, with room for improvement.  
        %An HPC domain expert rated the generated answers, against the above criteria. \textit{On average, the responses were rated highly coherent and relevant to the questions, indicating strong alignment with the input queries and well-structured output. Factual accuracy received a slightly lower mean score, suggesting occasional inconsistencies or minor hallucinations; the completeness score reflects generally sufficient coverage of expected information, though with some room for improvement in capturing all relevant details.}\\
        %Along with human evaluation by our Subject Matter Experts (SMEs), 
        Additionally, we used state-of-the-art Large Language Model GPT-4o to evaluate the generated answers with the same criteria as the domain experts on a randomly sampled 50 QA pairs (Table \ref{tab:human-llm-eval}).
        The results show high high relevance and coherence metrics value but relatively lower on factual accuracy and completeness. 
        %\textit{We can clearly see that our responses are high on relevance and coherence, and a little low on factual accuracy and completeness on the sample set. This is clearly because of the conciseness of our answers which results in more information to be desired in the generated responses.} \\
        
        \textbf{Finding 1:} \textit{The multimodal \textit{IR} module performs well with shorter Q\&A, generating relevant and correct responses; however  there is room for improvement in handling long-form Q\&A. The results underscore the importance of extensive evaluation.} 
        %Our answers could be further improved by the fine-tuned version of our RAG model on HPC questionnaires which we intend to do next. Also, the multimodal information retrieval could be better with targeted post-processing and updated/larger models (in terms of embedding, similarity-based retrieval, and re-ranking).\\

        \input{tables/document_rag_table_and_images}
                

       
     
    \input{tables/document_RAG_human_eval}
    
    %\subsubsection{Telemetry}
    \subsection{Descriptive Analytics}
        % Preamble of predictive analytics I. \loremipsum{\text odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim }
        % Telemetry module evaluation metrics goes here, 3 columns.
        % Overall description
        The \textit{DA} module is primarily based on the conversion of natural language into SQL for operational analytics tasks for insights on the past datasets. 
        \input{tables/telemetry_eval}
        For evaluation, we compare 453 generated SQL statements with the ground-truth counterparts, grouping them by keywords and functions (shown in~Table~\ref{tab:telemetry_results_key_fun}). 
        Using the evaluation method described in Section~\ref{sec:design}.2, the model generated correct SQL for 396 data points.  
        Grouping help us ascertain the quality of the model based on complexity of SQL. Complex of SQL depends on number of \textit{keywords} and type of \textit{keywords}. 
        Table~\ref{tab:telemetry_results_key_fun} lists 30 different SQL patterns, showing the number of questions per pattern and the count of correctly converted natural language queries. Some patterns exhibit high matching scores, while others, particularly those in rows 23 and 25, have significantly lower success rates.  
        
        We further analyze these \textit{SQL Functions and Keywords}, which are compound patterns of multiple keywords, by decomposing them into atomic patterns. This involves extracting and analyzing individual keywords.

        The plot in Figure~\ref{figs:telemetry_group_accuracy} shows the model performance based on the atomic \textit{Keywords} vs. accuracy. Atomic patterns, which involve single keywords reveal that functions, such as \textit{LIMIT} and \textit{ORDER BY}, have the highest accuracy, while \textit{EXTRACT} \& \textit{FRACTION} have the lowest accuracy percentage.  \textit{EXTRACT} is a SQL function to extract used to extract absolute time component, such as the hour of the day ($0$-$23$), or week of the year ($0$-$53$), independent of the year. 
        We then group these keywords into six categories based on the type of SQL function types: \textit{selection \& retrieval}, \textit{aggregation functions}, \textit{data manipulation}, \textit{conditional logic}, \textit{joining \& grouping}, and \textit{ordering}.
        The plot in Figure~\ref{figs:telemetry_group_accuracy} also illustrates the performance of the model'sperformance across these six categories.We observe that the data manipulation functions are relatively complex and more challenging to generate. 
 
        \begin{figure}[t]
          \centering
          \includegraphics[width=\linewidth]{figs/telemetry_group.png}
          \caption{SQL keywords wise performance of the telemtery module. 
          The keywords are classified into six groups based on the type of SQL keywords. }
          %\Description{Description of the image}
          \label{figs:telemetry_group_accuracy}
        \end{figure}
        
        The number of table joins or combined dataset sources is a crucial aspect of analytical questions. Increasing the number of joins can enhance query complexity and may affect the model performance. Figure~\ref{figs:telemetry_join_accuracy} illustrates the model's accuracy based on the number of joins. The red bar indicates number of questions for each 'join' category, while blue bar shows the percentage accuracy for the respective number of joins. 
        We observe that model performs well across all the three categories, maintainin at least 85\% accuracy. This is significant, as the HPC ODA tasks often require merging data from multiple tables, and the model strong performance in handling joins is encouraging.  
        
        \begin{figure}[t]
          \centering
          \includegraphics[width=\linewidth]{figs/telemetry_join.png}
          \caption{Model performance based on the number of data source involved.}
          \label{figs:telemetry_join_accuracy}
        \end{figure}

        Generating SQL is not a typical text-to-text generation problem for language models. We compare the general purpose state of the art propriety \textit{OpenAI-4o} model with open-weight \textit{Llama-3 model} model fine-tuned for SQL. The  \textit{OpenAI-4o} model is significantly larger than 8-billion parameter \textit{Llama-3} model we employed. Figure~\ref{fig:telemetry_model_comparision} compares the 3 models: base \textit{Llama-3-8b} model, \textit{OpenAI-4o} model and \textit{Llama-3} 8b model fine-tuned for SQL datasets. While \textit{OpenAI-4o} model outperforms the base \textit{Llama-3} model, the fine-tuned \textit{Llama-3} model exhibits significantly better accuracy than the \textit{OpenAI-4o} model for SQL tasks. 
        %comparing two general-purpose language models i.e. base Llama with \texttt{4o}, we observe that \texttt{4o} model accuracy is far better than the \texttt{Llama-3} model. However, when the \texttt{Llama-3} model is fine-tuned on SQL datasets the smaller fine-tuned \texttt{Llama} model exhibit significantly better accuracy compared to \texttt{4o} model.\\
        
        \textbf{Finding 2: } \textit{The accuracy of the analytical model may depend on the complexity of the SQL being generated. However, we observed that the number of joins did not significantly affect model performance. Users should be cognizant of these nuances when performing analytics with these tools.}
        
        \textbf{Finding 3: } \textit{We demonstrate that for specialized tasks, such as analytics, smaller, fine-tuned models can outperform larger, general-purpose models.}
        
        \begin{figure}[t]
          \centering
          \includegraphics[width=\linewidth]{figs/telemetry_model_comparisions.png}
          \caption{Performance of three models. (0: Aggregation functions, 1: Conditional logic,
          2: Data manipulations, 3: Joining and Grouping, 4: Ordering, and 5: Selection and retrieval)}
          %\Description{Description of the image}
          \label{fig:telemetry_model_comparision}
        \end{figure}        
        
    \subsection{Predictive Analytics}
        In this section, we evaluate the performance of the predictive analytics module, divided into two parts based on the two sub-modules. The first part evaluates the parsing of user questions, and their translation into a structured output by LLM. The second part is evaluates the regression model using various error metrics.
        \begin{figure}[t]
          \centering
          \includegraphics[width=0.7\linewidth]{figs/prediction_eval_llm.png}
          \caption{Performance of the LLM model for translating user questions into the input and output feature for the prediction model }
          \label{figs:prediction_llm_eval}
        \end{figure}    
        
        For the evaluation of the natural language parsing, we observe the LLM accuracy in handling four input features and the output feature, as shown in Figure \ref{figs:prediction_llm_eval}.  The model achieves $100\%$ accuracy for two  input features (node count, utilization type) and above $79\%$ accuracy for the remaining two (domain, time). In case of choosing domains, model chooses some irrelevant domain along with the correct domain, which we consider inaccurate, and thus the accuracy drops. Similarly, for the runtime of the job, the model sometimes struggle converting minutes to seconds. In identifying the output feature, the model acheives $90\%$ accuracy. The only errors that have been observed is that in some of the power prediction questions, the model suggests energy as the output feature.   

         \input{tables/predictive_eval}

        \begin{figure}[h]
          \centering
          \includegraphics[width=\linewidth]{figs/prediction_rmse_mixed_scaler_four_targets_utilization_type.png}
          \caption{Performance (RMSE) of the \textit{regression}  submodule by utilization type for different output features: (a) GPU Power Max, (b) CPU Memory Power Max, (c) Node Power Mean, (d) Node Temperature Max, (e) Total Node Energy.}
          \label{figs:prediction_rmse_utilization}
        \end{figure}
        
        For the \textit{regression} submodule evaluation, we report all 
        error metrics for our test data for individual output features in Table \ref{tab:prediction_regression}. We observe that the temperature feature has the lowest error of $8\%$. For the power and energy features, the model shows $65\%$ to $94\%$ accuracy depending on the output feature variable. We also observe how the model performs corresponding to the input feature values. For the jobs utilizing GPUs, it show higher RMSE compared to the jobs running on CPUs given in Figure \ref{figs:prediction_rmse_utilization}. Next, we observe how the model performs for each of the science domains given in Figure \ref{figs:prediction_rmse_domain}. We observe that for the GPU Power or Temperature feature the model performs similarly for all of the domains. In case of the Node Power, and Node Energy we see the performance drop for a few domains namely, Fluid Dynamics (CFD), and Physics for Node Power. In addition, Nuclear Fuel, Fusion Engineering, Astro Physics have higher errors compared to the rest of the domains while predicting Total Node Energy.   \\

        \textbf{Finding 4: }\textit{%The LLM achieves $100\%$ accuracy in \texttt{query-interpretation} submodule when the input features are node count and utilization type, and over $79\%$ accuracy for domain and time, with errors mainly due to selecting extra domains or incorrect unit conversions. Output feature identification is $90\%$ accurate, with occasional confusion between power and energy features.
        Again, the Llama model demonstrates high performance for the "specific" task of generating structured 'json' datasets.}

        \textbf{Finding 5: }\textit{Predictive models, like the regression model we have demonstrated, can be a modality in operational data representing a summary of past data and can be effectively synthesized into the analysis thanks to the EPIC's modular capabilities.}

        
        

        
        \begin{figure}[t]
          \centering
          \includegraphics[width=\linewidth]{figs/prediction_rmse_mixed_scaler_four_targets_domain.png}
          \caption{~Performance (RMSE) of the  \textit{regression} submodule by science domains for different output features. }
          \label{figs:prediction_rmse_domain}
        \end{figure}






        
        % \begin{figure}[t]
        %   \centering
        %   \includegraphics[width=\linewidth]{EPIC/figs/prediction_model.png}
        %   \caption{\naw Performance of the prediction model.}
        %   \label{figs:template_single}
        % \end{figure}
 
       
    
    \subsection{Routing, Reasoning, and Synthesis}
    \label{subsec:eval:routing}
        
        In this section, we evaluate the routing, reasoning, and synthesis capability of the high-level agentic tool calling loop.  For this, we have developed an evaluation loop that performs end-to-end tests with test examples that aims for varying degrees of routing and synthesis required by the examples framing it as a classification problem.
        
        In simple cases, the examples would require a single instance of delegation representing RAG – information retrieval, SQL – descriptive analytics, or PRD – predictive analytics as classes.  More complicated cases would demand reasoning and sequencing of multiple capabilities represented as additional four classes: RAG+SQL, RAG+PRD, SQL+PRD, and RAG+SQL+PRD). Additionally, we consider a class which none of the lower-level modules are involved (i.e., greetings in a conversation). The evaluation loop scores both the accuracy of the call and the synthesized result. We employed total 181 examples in which simple case examples are coming from other per-capability evaluations (60 examples in total) and the complex ones were dedicated just for this evaluation.

        Fig.~\ref{figs:routing_eval} shows the accuracy of correct tool routing per classes in a confusion matrix. With an F1-score of 0.77 at the macro level, we could confirm high accuracy for each class except for RAG+SQL+PRD. The top-level model is capable of reasoning about the necessary steps to fulfill the query with proper delegation. Further, Fig.~\ref{figs:end_to_end} shows the quality of the synthesized result from the 181 examples evaluated by subject matter experts using the Likert scale. With a mean score of 3.89 overall, we confirm EPIC can return acceptable results except for classes that involve predictions (PRD, SQL+PRD, RAG+SQL+PRD).

        \textbf{Finding 6: }\textit{The top-level query processing module leveraging proprietary foundation models are capable of handling complex analysis questions by understanding the steps to fulfill the user query in an autonomous fashion.}


        %% Original code and data in latex.overleaf.gov : Code/router_eval/routing_eval.py
        \begin{figure}[t]
          \centering
          \includegraphics[width=\linewidth]{figs/routing_eval.pdf}
          \caption{Confusion matrix of the routing capability reasoned by the top-level model yielding an F1 score of 0.77}
          \label{figs:routing_eval}
        \end{figure}

        %% Original code and data in latex.overleaf.gov : Code/router_eval/end_to_end.py
        \begin{figure}[t]
          \centering
          \includegraphics[width=\linewidth]{figs/end_to_end.pdf}
          \caption{End-to-end human evaluation: performed on 181 high-level questions, reporting mean Likert scale per class (dot) and their distribution}
          \label{figs:end_to_end}
        \end{figure}
    
    \subsection{Inference Cost Evaluation}
        Advanced LLM models, can incur significant costs when running inference tasks. Therefore, cost evaluation is a critical component when designing and implementing LLMs. 
        We compare the cost of inference on the \textit{Llama-3-8B} model when hosted by a cloud service provider and accessed through a serverless API. 
        We use the number of tokens and the cost per token as metrics. 
        Tokens can be words, parts of words, or individual characters, and language models break down text into these tokens to understand and generate text.
        We compare the costs of serverless APIs from OpenAI and the Llama-3 8B model. The per-token cost for OpenAI is \$0.0000025 for input tokens and \$0.000010 for output tokens. For the Llama-3 8B model, the per-token cost is \$0.000003 for input tokens and \$0.0000061 for output tokens.
        
        In Figure~\ref{figs:cost_eval_tokens}(a), we show the total number of tokens used by all the questions in \textit{DA} module evaluation tasks. Input tokens are calculated from queries asked to the models and output tokens are generated by response of the models. We observe that, for both models have more input token than output token. Also number of tokens of OpenAI model is similar to Llama models. However, the cost of using these tokens is significantly higher for OpenAI models (shown in Figure~\ref{figs:cost_eval_tokens}(b)). \\
        \textbf{Finding 7: } \textit{The cost of operating Llama model is 8.3 times less than that of OpenAI-4o models for input tokens and likewise, for output tokens, cost of Llama model is  19.1 times less compared to OpenAI-4o model. Thus, we demonstrate that the relatively smaller Llama models can do better or comparable in terms of performance evaluation at a fraction of the cost.}  
    
        \begin{figure}[t]
              \centering
              \includegraphics[width=\linewidth]{figs/cost_eval_tokens.png}
              \caption{Figure illustrating comparison of token count \& inference cost of OpenAI and Llama models.}% (a) Comparison of input and output tokens. (b) The respective cost of inference of the two models.}
              \label{figs:cost_eval_tokens}
        \end{figure}

==> EPIC_arXiv/txt/06_discussion.tex <==
\iffalse
\section{Discussion}
\label{sec:discussion}
    \ahmad~
    %Discussion 1 column    
    Discussions III. \loremipsum{\text odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing convallis aenean et tortor at risus viverra adipiscing
    }  

    \ahmad~Discussions III. \loremipsum{\text odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing convallis aenean et tortor at risus viverra adipiscing
    }

    \ahmad~Discussions IV. \loremipsum{\text odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing
    }    

\fi

==> EPIC_arXiv/txt/06_related.tex <==

\section{Related Works}
\label{sec:relatedWorks}


\woong()
\loremipsum{\textbf{100-words}
odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing at in tellus integer feugiat scelerisque varius morbi enim nunc faucibus a pellentesque sit amet porttitor eget dolor morbi non arcu risus}

\loremipsum{\textbf{100-words}
odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing at in tellus integer feugiat scelerisque varius morbi enim nunc faucibus a pellentesque sit amet porttitor eget dolor morbi non arcu risus}

==> EPIC_arXiv/txt/07_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
    %\ahmad~
With the increasing operational complexity, ODA has become one of the key components of achieving high operational efficiency in HPC. However, it has hardly been a trivial endeavor for HPC centers to make impact with data. There is an unmistakable gap between data and insight mainly bottlenecked by the complexity of handling large amounts of data from various sources while fulfilling multi-faceted use cases targeting many different audiences. We observe that the ODA is bottlenecked by manual data exploration efforts, campaigns, analysis, synthesis, interpretation, and visualization of data.
%These tasks, which are crucial for making impact has largely been static with a steep learning curve due to the multi-disciplinary nature of ODA. 
    
To solve this “last mile” issue of data, we have presented the design and implementation of EPIC, a new capability that accelerates data exploration and analysis tasks in HPC ODA systems by leveraging the emerging capabilities of generative AI. 
EPIC’s dynamic, modular design enables it to adapt to evolving analytics tasks. 
%Posing the question of “what is the role and impact of generative AI in the HPC operational environment?”, 
We have found that the emerging reasoning and synthesis capabilities large language models can automate the synthesis multiple modalities of operational data; 1) unstructured HPC domain knowledge – text, image, and tables, 2) structured traditional tabular data, and 3) consumption of models of data for predictions.  Further, we have found that such reasoning and synthesis can be integrated in existing HPC ODA systems in a cost-effective, modular and extendible way by integrating generative AI by leveraging multiple agentic loops collaborating in a hierarchical way.

Through extensive evaluations, we have demonstrated that these capabilities are effective in handling each modality handling various ODA tasks. Also, these tasks would be reasoned about and be executed in an automated workflow to fulfill complex queries.
%With a prototype implementation spanning three systems, EPIC is currently limited to a fixed set of domain knowledge, tabular data and a static model.
As future work, we aim extend this system to handle a wider array of tasks by introducing more lower-level capabilities better integrated with the real-time nature of ODA systems. Also, we aim to further explore and enhance the trustworthiness and reliability of end-to-end agentic approaches by tackling the problem of system evaluations.

==> figs/sql_comparision.tex <==
%% Template for a page-wide figure
\begin{figure}[t]
  \centering
  
  \includegraphics[width=\linewidth]{EPIC/figs/sql_comparision.png}
  \caption{The two SQL statements (a) and (b) generate exactly same data despite being different.}
  %\Description{Description of the image}
  \label{fig:sql_comparision}
\end{figure}


==> tables/routing_eval.tex <==
\begin{table}
  \caption{\woong~Evaluation of Routing, Reasoning and Synthesis}
  \label{tab:routing_eval}
  %% Footnotesize if a much smaller font is needed
  %\footnotesize
  \centering
  \begin{tabular}{ccccc}
    
    \toprule
      colA & colB & colC & colD  \\
    \midrule
      \multirow{3}{*}{\rotatebox{90}{\parbox{1cm}{\centering Query Parsing}}}& \O & 1 in 1,000 & hello  & world  \\
      & \O & 1 in 1,000 & hello  & world  \\
      & \O & 1 in 1,000 & hello  & world  \\
    
    \midrule

  \multirow{3}{*}{\rotatebox{90}{\parbox{1cm}{\centering Prediction model}}}& \O & 1 in 1,000 & hello  & world  \\
      & \O & 1 in 1,000 & hello  & world  \\
      & \O & 1 in 1,000 & hello  & world  \\
    
  \bottomrule
\end{tabular}
\end{table}

==> txt/06_discussion.tex <==
\iffalse
\section{Discussion}
\label{sec:discussion}
    \ahmad~
    %Discussion 1 column    
    Discussions III. \loremipsum{\text odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing convallis aenean et tortor at risus viverra adipiscing
    }  

    \ahmad~Discussions III. \loremipsum{\text odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing convallis aenean et tortor at risus viverra adipiscing
    }

    \ahmad~Discussions IV. \loremipsum{\text odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing
    }    

\fi

==> txt/06_related.tex <==

\section{Related Works}
\label{sec:relatedWorks}


\woong()
\loremipsum{\textbf{100-words}
odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing at in tellus integer feugiat scelerisque varius morbi enim nunc faucibus a pellentesque sit amet porttitor eget dolor morbi non arcu risus}

\loremipsum{\textbf{100-words}
odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing at in tellus integer feugiat scelerisque varius morbi enim nunc faucibus a pellentesque sit amet porttitor eget dolor morbi non arcu risus}
